Optimistic Prediction of Synchronization-Reversal Data Races

Dynamic data race detection has emerged as a key technique for ensuring reliability of concurrent software in practice. However, dynamic approaches can often miss data races owing to nondeterminism in the thread scheduler. Predictive race detection techniques cater to this shortcoming by inferring alternate executions that may expose data races without re-executing the underlying program. More formally, the dynamic data race prediction problem asks, given a trace \sigma of an execution of a concurrent program, can \sigma be correctly reordered to expose a data race? Existing state-of-the art techniques for data race prediction either do not scale to executions arising from real world concurrent software, or only expose a limited class of data races, such as those that can be exposed without reversing the order of synchronization operations. In general, exposing data races by reasoning about synchronization reversals is an intractable problem. In this work, we identify a class of data races, called Optimistic Sync(hronization)-Reversal races that can be detected in a tractable manner and often include non-trivial data races that cannot be exposed by prior tractable techniques. We also propose a sound algorithm OSR for detecting all optimistic sync-reversal data races in overall quadratic time, and show that the algorithm is optimal by establishing a matching lower bound. Our experiments demonstrate the effectiveness of OSR on our extensive suite of benchmarks, OSR reports the largest number of data races, and scales well to large execution traces.

==> algos/algo-abstract-graph-incremental.tex <==
%!TEX root=../main.tex

\begin{algorithm}
\caption{Checking if $\redgraph_S$ is cyclic}
\algolabel{cyclic-abstract-graph}
\myproc{\absCycle{$S$}}{
	$\redvertices, \rededges \gets \varnothing$ \\
	\For{$\lk \in \locks{\trace}$}{
		\If{$\exists \; \acqO{\lk}, \last{\rel(\lk)} \in S$}{
			$\redvertices \gets \redvertices \cup \set{\acqO{\lk}, \; \last{\rel(\lk)}}$ \\
			$\rededges \gets \rededges \cup \acqO{\lk} \rightarrow \last{\rel(\lk)}$
		}
	}
	\For{$u \in \redvertices$}{
		$Succ \gets$ $getSuccessors(u, S)$ \\
		\For{$v \in \redvertices$, s.t. $v \neq u$}{
			\If{$Succ[\ThreadOf{v}] \thAfter v$}{
				$\rededges \gets \rededges \cup u \rightarrow v$
			}
		}   
	}
	$\redgraph \gets (\redvertices, \rededges)$ \\
	\Return{$\redgraph$ has a cycle}
}    
\end{algorithm}


==> algos/algo-closure-incremental.tex <==
%!TEX root=../main.tex

\begin{algorithm}
    \caption{computeOSR($e_1$, $e_2$, $\SSP{e_1', e_2}$)}
    \label{algo:calcOSRIncre}
    \KwData{Two conflicting events $e_1$, $e_2$ and a previous \ssp event set $\SSP{e_1', e_2}$ with $e_1' \thAfter e_1$} 
    \KwResult{$\SSP{e_1, e_2}$}
    $S \; \leftarrow \; \SSP{e_1', e_2}$ \\ 
    $S \; \leftarrow S \cup \TLC{\prev{\trace}{e_1}} \cup \TLC{\prev{\trace}{e_2}}$ \\
    \While{$S$ changes}{
        \If{$\exists \; \lk$  $\in$ $\locks{\trace}$, $\acq(\lk)$ $\in$ $S$, $\match{\trace}{\acq(\lk)} \notin S$ }{
            \If{$e_1, e_2 \notin \cap$ $\TLC{\match{\trace}{\acq(\lk)}}$}{
                $S$ $\leftarrow$ $S$ $\cup$ $\TLC{\match{\trace}{\acq(\lk)}}$ \\
            }
        }
    }
    \Return{$S$} \\
\end{algorithm}

==> algos/algo-closure-single.tex <==
%!TEX root=../main.tex

\begin{algorithm}
    \caption{Compute OSRClosure for given $e_1, e_2$}
    \label{algo:computeOSR}
    \SetKwProg{handler}{Procedure}{}{}
    \handler{computeOSR($e_1$, $e_2$)}{
        $S \; \leftarrow \TLC{\prev{\trace}{e_1}} \; \cup \; \TLC{\prev{e_2}}$ \\
        \While{$S$ changes}{
	        \If{$\exists \lk \in \locks{\trace}$, $\acq(\lk) \in S$, $\match{\trace}{\acq(\lk)} \notin S$ }{
	            \If{$e_1, e_2 \notin \cap$ $\TLC{\match{\trace}{\acq(\lk)}}$}{
	                $S$ $\leftarrow$ $S$ $\cup$ $\TLC{\match{\trace}{\acq(\lk)}}$ \\
	            }
	        }
        }
        \Return $S$
    }
\end{algorithm}

==> algos/algo-detect-races-given-two-events.tex <==
%!TEX root=../main.tex

\begin{algorithm}
\caption{Given two conflicting events and a previous event set $S$, do incremental race detection based on $S$}
\algolabel{check-race-given-two-events}
% \KwData{Two conflicting events $e_1$, $e_2$ and $\SSP{e_1', e_2}$ with $e_1' \thAfter e_1$} 
% \KwResult{Determine if ($e_1$, $e_2$) is a race}
\myproc{checkRace($e_1$, $e_2$, $S$)}{
    $S \gets$ $computeOSR(e_1, e_2, \SSP{e_1', e_2})$ \\
    \eIf{$buildGraphAndCheckCycles(S)$}{
        Declare a race
    }{
        Declare no race
    }
}
\end{algorithm}

==> cycleDetectionOld.tex <==
\noindent
Given the event set and well-defined edges, one may simply linearize the SSP event set with graph-based algorithms like topological sort. We also implemented a similar version, but it turns out to be extremely slow. The reason being that we cannot do cycle detection incrementally. To efficiently detect cycles, we decide to do some approximations that will increase the scalibility of SSP, without compromising the prediction power too much.

\noindent
At a high level, we try to make the conditions stronger than`there is no cycle in SSP event set, i.e. if the new condition is satisfied, we can guarantee there is no cycle in SSP event set, but it could be possible that the SSP event set contains no cycle, but it doesn't meet the conditions. The implication, in terms of data races, is  that we may detect fewer races than the previous SSP with faster speed. Another intuition is that from the previous SSP cycle detection experience, we already know it's expensive to do topological sort on graphs. Therefore, we want to transfer the reasoning about existence of a cycle into reasoning about the membership of an event in an event set. This is potentially easier, because our events are downward closed with respect to thread-order and membership question corresponds to a vector-timestamp comparison (which can be done in $O(1)$ time). 

\noindent
\textbf{Conflict Closure: } For a trace $\trace$, and an event $e$ in $\trace$, the conflict closure of $e$, denoted $\Conf{e}$ is the smallest set of events such that
\begin{enumerate}
    \item $e$ $\in$ $\Conf{e}$
    \item $\forall$ event $e'$ $\in$ $\Conf{e}$, $\forall$ event $e''$ $\in$ $\trace$ and $e''$ $\thAfter$ $e'$, we have $e''$ $\in$ $\Conf{e}$.
    \item $\forall$ event $e'$ $\in$ $\Conf{e}$, if $e'$ is a write operation on $x$, then $\forall$ $\writeOp{x}$, $\readOp{x}$ $\in$ $\trace$, s.t. $\writeOp{x}$ or $\readOp{x}$ $\trAfter$ $e'$, we have $\writeOp{x}$ or $\readOp{x}$ $\in$ $\Conf{e}$.

    \item $\forall$ event $e'$ $\in$ $\Conf{e}$, if $e'$ is a read operation on $x$, then $\forall$ $\writeOp{x}$ $\in$ $\trace$, s.t. $\writeOp{x}$ $\trAfter$ $e'$, we have $\writeOp{x}$ $\in$ $\Conf{e}$.
\end{enumerate}
\begin{lemma}
    $\forall$ $e'$ $\in$ $\Conf{e}$, we have $\Conf{e'}$ $\subseteq$ $\Conf{e}$.
\end{lemma}

\noindent
\textbf{Intuition for cycle detection.} Here we briefly introduce how to simplify the cycle detection with quasi order defined above. The first observation we make is that any cycle involves at least one backward edge (edges from event appears later in $\trace$ to event appears earlier in $\trace$). However, reasoning about multiple backward edges is challenging and as a result, we restrict the number of backward edges to be at most one. And we note that if it exists, this backward edge can be represented as $\acqO{l}$ $\gets$ $\last{\rel{l}}$, where $\acqO{l}$ is the unique open acquire on lock $l$. Then any cycle must contain this edge, as it is the only backward edge in the whole graph. Then we try to compute a set $X$, s.t. this set contains all events that have a path from itself to $\last{\rel{l}}$. We argue that it's sufficient to check whether $\acqO{l}$ $\in$ $X$, because if there is a cycle, then there must exist a path from $\acqO{l}$ to $\last{\rel{l}}$, thus we should have $\acqO{l}$ $\in$ $X$. The intuition is formalize below.

~\\ \textbf{Predecessor Set: } Let $S$ denotes the SSP event set of $e_1, e_2$, and the predecessor set $\Pred{e_1}{e_2}$ is defined as
\begin{equation}
    \Pred{e_1}{e_2} = \bigcup\limits_{\rel{l}\; \in \; S \;} \Conf{\rel{l}} \nonumber
\end{equation}
$\Pred{e_1}{e_2}$ should contain all events that have a path from themselves to $\last{\rel{l}}$ in $\POrder$. We now first make a simple observation about predecessor sets.
\begin{proposition}
    $\forall$ events $e_1$, $e_2$ and $e_2'$, if $e_2$ $\thAfter$ $e_2'$, then we have $\Pred{e_1}{e_2}$ $\subseteq$ $\Pred{e_1}{e_2'}$.
\end{proposition}
\noindent
We now state our main observation formally:
\begin{lemma}
    \lemlabel{fast-cycle-detection}
    Let $\trace$ be a trace, $e_1$, $e_2$ be two conflicting events in $\events{\trace}$, if the one of the following conditions hold for every lock $l$ (referred to by the predicate $\ACyclic{e_1}{e_2}$), then the quasi order $\POrder$ contains no cycle in $\SSP{e_1}{e_2}$.
    \begin{enumerate}[label=(\arabic*)]
    \item There is no open acquire on $l$ in $\SSP{e_1}{e_2}$, or 
    
    \item There is an open acquire $\acqO{l} \in \SSP{e_1}{e_2}$, s.t. $\forall \; \rel{l} \in \SSP{e_1}{e_2}$, we have $\rel{l} \trAfter \acqO{l}$ (i.e. no backward edges), or
    
    \item There is an open acquire $\acqO{l} \in \SSP{e_1}{e_2}$, s.t. $\exists \; \rel{l} \in \SSP{e_1}{e_2}, \acqO{l} \trAfter \rel{l}$, and $\acqO{l}$ $\notin$ $\Pred{e_1}{e_2}$. And $l$ is the only lock satisfying this condition, or
    
    \item There is an open acquire $\acqO{l} \in \SSP{e_1}{e_2}$, s.t. $\exists \; \rel{l} \in \SSP{e_1}{e_2}, \acqO{l} \trAfter \rel{l}$, and $\forall e, s.t. \acqO{l} \thAfter e$, $e$ is an acquire event.
    \end{enumerate}
\end{lemma}

\noindent
Assuming $\ACyclic{e_1}{e_2}$ holds, we prove $\POrder$ is acyclic by showing every backward edge cannot form a cycle. Noticing that backward edges can only appear in condition (3) and (4). 

\noindent
Firstly, we show all backward edges of lock $l$ in condition (4) cannot form a cycle. Assuming $\last{\rel{l}} \rightarrow \acqO{l}$ is in a cycle, there must be a path starting from $\acqO{l}$ to $\last{\rel{l}}$. However, the only type of edge starting from $\acqO{l}$ is Thread Order. This means $\acqO{l}$ can only point to another acquire event in the same thread. Following the same analysis procedure, any path starting from $\acqO{l}$ cannot contain events from another thread, thus it's impossible to have such paths in $\SSP{e_1}{e_2}$.

\noindent
Secondly, if there is a lock $l$ in $\SSP{e_1}{e_2}$ satisfying condition (3),  we show if the edge $\last{\rel{l}} \rightarrow \acqO{l}$ exists in any cycle, then we should conclude $\acqO{l} \in \Pred{e_1}{e_2}$. And since we observed $\acqO{l} \notin \Pred{e_1}{e_2}$, $(\last{\rel{l}}, \acqO{l})$ is not in any cycle. Assuming there is a cycle containing $\last{\rel{l}} \rightarrow \acqO{l}$, according to the definition of a cycle, there is a path from $\acqO{l}$ to $\last{\rel{l}}$. As all backward edges in condition (4) cannot exist in any cycle, we have $\last{\rel{l}} \rightarrow \acqO{l}$ is the only backward edge in the cycle, all other edges in the cycle are forward edge, i.e. starting from event appeared earlier in $\trace$ to event appeared later in $\trace$.

\noindent
We label events in this cycle as following: starting from $\last{\rel{l}}$,
\begin{enumerate}
    \item For the event that directly forwards to $\last{\rel{l}}$ by an edge, we define it as $f_1$.

    \item For an event that directly forwards to $f_i$, $i \ge 1$, we define it as $f_{i+1}$.
\end{enumerate}
\noindent
There is a figure below showing the general picture of a cycle.

~\\ Then we inductively prove that $\forall$ $f_i$ with $i \ge 1$, we should have $f_i$ $\in$ $\Pred{e_1}{e_2}$.
\begin{enumerate}
    \item Firstly, we have $f_1$ $\in$ $\Pred{e_1}{e_2}$, because the edge pointing to $\last{\rel{l}}$ can only be Thread Order.
    \item For given integer $i$, if $\forall$ $j < i$, we have $f_j$ $\in$ $\Pred{e_1}{e_2}$, then we prove $f_i$ $\in$ $\Pred{e_1}{e_2}$. As $\Pred{e_1}{e_2}$ is a Conflict Closure, we have $\Conf{f_{i-1}}$ $\subseteq$ $\Pred{e_1}{e_2}$. Consider the type of edge $f_i \rightarrow f_{i-1}$ as following.

    \begin{enumerate}
        \item If the edge of $f_i \rightarrow f_{i-1}$ is Thread Order. Then we have $f_{i}$ $\in$ $\Conf{f_{i-1}}$ $\subseteq$ $\Pred{e_1}{e_2}$.
        \item If the edge of $f_i$ $\rightarrow$ $f_{i-1}$ is Read-From Order. Then we have $f_{i-1}$ is a read operation and $f_i$ is a write operation and they operate on the same variable. In this case, we must have $f_{i}$ $\in$ $\Conf{f_{i-1}}$ $\subseteq$ $\Pred{e_1}{e_2}$. And similarly we can prove for $f_i$ $\rightarrow$ $f_{i-1}$ being Write-Write or Read-Write.
        \item If the edge of $f_i$ $\rightarrow$ $f_{i-1}$ is lock-semantics order, then $f_i$ must be a release event and $\Pred{e_1}{e_2}$ should contain all release events in $\SSP{e_1}{e_2}$ \ucomment{Not acording to your definition of Pred}. This also applies for edges from Open Acquires Order.
    \end{enumerate}
\end{enumerate}


\begin{figure}[H]
    \centering 
    \includegraphics[width=0.5\textwidth]{./figures/demo-cycle.png}
    \caption{Demo of a cycle} 
    \label{Fig.main2} 
\end{figure}


In summary, we inductively proved that all events in the cycle trace before $\last{\rel{l}}$ should exist in the set $\Pred{e_1}{e_2}$, thus $\acqO{l}$ $\in$ $\Pred{e_1}{e_2}$. And since we require $\acqO{l}$ $\notin$ $\Pred{e_1}{e_2}$, this eliminates the possibility of any cycles. We have two further optimizations to $\Pred{e_1}{e_2}$. Note that the $\Pred{e_1}{e_2}$ is not necessarily a subset of $\SSP{e_1}{e_2}$, and we must have $\acqO{l}$ $\in$ $\SSP{e_1}{e_2}$. Therefore, it's equivalent to transfer the condition of $\acqO{l}$ $\notin$ $\Pred{e_1}{e_2}$ to $\acqO{l}$ $\notin$ $\Pred{e_1}{e_2} \cap \SSP{e_1}{e_2}$.

% \begin{minipage}{\textwidth}
% 	\centering
% 	\begin{minipage}[t]{0.45\textwidth}
% 		\centering
% 		\begin{table}[H]\centering
% 			\begin{tabular}{|c|cc|}
% 				\hline $\,$ & $t_1$             & $t_2$       \\
% 				\hline 1    & $\acq{l_1}$       & $\,$      \\
% 				2           & $\writeOp{x}$     & $\,$      \\
% 				3           & $\rel{l_1}$       & $ $      \\
% 				4           & $\acq{l_2}$       & $ $       \\
% 				5           & $\readOp{x}$      & $ $       \\
% 				6           & $\rel{l_2}$       & $ $       \\
% 				7           & $\,$              & $\acq{l_1}$       \\
% 				8           & $\,$              & $\writeOp{x}$       \\
% 				9           & $\,$              & $\rel{l_1}$       \\
% 				10          & $\,$              & $\acq{l_2}$      \\
%                     11          & $\,$              & $\readOp{x}$     \\
% 	            12          & $\,$              & $\rel{l_2}$       \\
%                 \hline
% 			\end{tabular}
% 			\caption*{\textbf{(a)} $(e_2, e_{11})$ is a race}
% 		\end{table}
% 	\end{minipage}
% 	\begin{minipage}[t]{0.45\textwidth}
% 		\centering
% 		\begin{table}[H]\centering
% 			\begin{tabular}{|c|cc|}
% 				\hline $\,$ & $t_1$             & $t_2$       \\
% 				\hline 
%                     1           & $\,$              & $\acq{l_1}$       \\
% 				2           & $\,$              & $\writeOp{x}$       \\
% 				3           & $\,$              & $\rel{l_1}$       \\
% 				4          & $\,$              & $\acq{l_2}$      \\
%                     5            & $\acq{l_1}$       & $\,$      \\
%                 \hline
% 			\end{tabular}
% 			\caption*{\textbf{(a)} witness $\reordering$}
% 		\end{table}
% 	\end{minipage}
% \end{minipage}

% ~\\ The second optimization is inspired by the example above. Firstly we compute the SSP event set to be \{$e_1$, $e_7$, $e_8$, $e_9$, $e_{10}$\} and we found this set is potentailly feasible. It also passes the first condition of only one backward edge $e_1 \gets e_9$. However, the $\Pred{e_1}{e_2}$ is computed to be \{$e_1$, $e_2$, $e_3$, $e_4$, $e_5$, $e_7$, $e_8$, $e_9$\} and after intersecting with SSP event set, we get \{$e_1$, $e_7$, $e_8$, $e_9$\}, which includes the open acquire event $e_1$, thus we have to declare no race. But a closer observation tells us it's not reasonable to include $e_1$ into $\Pred{e_2}{e_{11}}$, because it is included by $e_5$ or $e_2$, which is in the $\Conf{e_8}$, and $e_5$ or $e_2$ don't even exist in the SSP event set. No other events can include $e_1$. Clearly we should not include $e_1$ into the $\Pred{e_2}{e_{11}}$, but unfortunately, to do a complete exclusion of such elements would be too complicated and we here present a very simple solution that would work for this situation.

% \begin{lemma}
%     Let $S = \Pred{e_1}{e_2} \cap \SSP{e_1}{e_2}$. If $\forall \; l \in \locks{\trace}$ and $\forall$ event $e \in S$, s.t. $\acqO{l} \thAfter e$, we have $e$ is an acquire event, then $\SSP{e_1}{e_2}$ contains no cycle, even if $\acqO{l} \in S$ and there are multiple backward edges in SSP event set. 
% \end{lemma}
% \noindent
% This inspires us to check whether all the events in $S$ thread after $\acqO{l}$ are acquires, if so we can still declare no race and this solves the problem for the above example. More importantly, if we assume the maximum number of continuous acquire event is a constant, then the above optimization can be implemented with $O(T)$ time complexity.

==> figures/NPHard-Construction-Old.tex <==
\begin{figure*}
\usetikzlibrary{calc}
\newcommand{\xdisposition}{0}
\newcommand{\ydisposition}{0}
\newcommand{\xtstep}{0.75}
\newcommand{\ytstep}{0.7}
\newcommand{\ybias}{-0.3 }
\newcommand{\xstep}{2.5}
\newcommand{\ystep}{-0.475}
\newcommand{\xtscale}{0.8}

\def \numevents{23.5}

\newcommand{\eventA}[4]{
\node[event, draw=black, fill=white] (A#1) at (#1*\xstep, #2*\ystep) {\footnotesize $#2(x_{#3})$};
%\node[] at (0*\xstep-\xtstep, {#1*\ystep}) {\small $#2(x_{#3})$};
}

\scalebox{0.95}{
\begin{tikzpicture}[thick,
pre/.style={<-,shorten >= 2pt, shorten <=2pt, very thick},
post/.style={->,shorten >= 3pt, shorten <=3pt,   thick},
seqtrace/.style={->, line width=2},
und/.style={very thick, draw=gray},
event/.style={rectangle, minimum height=0.8mm, minimum width=15mm,  line width=1pt, inner sep=0.5,},
virt/.style={circle,draw=black!50,fill=black!20, opacity=0}]
\footnotesize


\node[] (G) at (-1.4*\xstep,6*\ystep) {\large  $G$};
\node[draw=black, circle, very thick] (1) at (-1.4*\xstep,9*\ystep) {\normalsize $1$};
\node[draw=black, circle, very thick] (2) at (-1.4*\xstep,7.5*\ystep) {\normalsize $2$};
\node[draw=black, circle, very thick] (3) at (-1.4*\xstep,10.5*\ystep) {\normalsize $3$};

\draw[-, very thick] (1) to (2);
\draw[-, very thick] (1) to (3);

\node[] (S11) at (0*\xstep,0) {\normalsize $\tau_1$};
\node[] (S12) at (0*\xstep,\numevents * \ystep) {};
\node[] (S21) at (2*\xstep,0) {\normalsize $\tau_2$};
\node[] (S22) at (2*\xstep,\numevents * \ystep) {};
\node[] (S31) at (1*\xstep,0) {\normalsize $\tau_3$};
\node[] (S32) at (1*\xstep,\numevents * \ystep) {};
\node[] (S41) at (3*\xstep,0) {\normalsize $\tau_4$};
\node[] (S42) at (3*\xstep,\numevents * \ystep) {};
\node[] (S51) at (4*\xstep,0) {\normalsize $\tau_5$};
\node[] (S52) at (4*\xstep,\numevents * \ystep) {};
\node[] (S61) at (5*\xstep,0) {\normalsize $\tau_6$};
\node[] (S62) at (5*\xstep,\numevents * \ystep) {};

\draw[seqtrace] (S11) to (S12);
\draw[seqtrace] (S21) to (S22);
\draw[seqtrace] (S31) to (S32);
\draw[seqtrace] (S41) to (S42);
\draw[seqtrace] (S51) to (S52);
\draw[seqtrace] (S61) to (S62);


\node[event, draw=black, fill=white] (11) at (0*\xstep, 1*\ystep + 0*\ybias) {$\acqSubs{1}{\ell_{\{1,2\}}}$};
\node[event, draw=black, fill=white] (12) at (0*\xstep, 2*\ystep + 0*\ybias) {$\acqSubs{1}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white] (13) at (0*\xstep, 3*\ystep + 0*\ybias) {$\writeOp{s_1}$};
\node[event, draw=black, fill=white] (14) at (0*\xstep, 4*\ystep + 0*\ybias) {$\readOp{z_1^1}$};
\node[event, draw=black, fill=white] (15) at (0*\xstep, 5*\ystep + 0*\ybias) {$\relSubs{1}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white] (16) at (0*\xstep, 6*\ystep + 0*\ybias) {$\relSubs{1}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white] (17) at (0*\xstep, 7*\ystep + 1*\ybias) {$\acqSubs{1}{\ell_{\{1,2\}}}$};
\node[event, draw=black, fill=white, line width=1.75] (18) at (0*\xstep, 8*\ystep + 1*\ybias) {$\writeOp{y_1^2}$};
\node[event, draw=black, fill=white] (19) at (0*\xstep, 9*\ystep + 1*\ybias) {$\readOp{z_1^2}$};
\node[event, draw=black, fill=white] (110) at (0*\xstep, 10*\ystep + 1*\ybias) {$\relSubs{1}{\ell_{\{1,2\}}}$};
\node[event, draw=black, fill=white] (111) at (0*\xstep, 11*\ystep + 2*\ybias) {$\acqSubs{1}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white] (112) at (0*\xstep, 12*\ystep + 2*\ybias) {$\writeOp{y_1^3}$};
\node[event, draw=black, fill=white] (113) at (0*\xstep, 13*\ystep + 2*\ybias) {$\readSubs{1}{x}$};
\node[event, draw=black, fill=white] (114) at (0*\xstep, 14*\ystep + 2*\ybias) {$\relSubs{1}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white] (301) at (0*\xstep, 15*\ystep + 2*\ybias) {$\writeOp{v_1}$};

\node[event, draw=black, fill=white] (21) at (2*\xstep, 1*\ystep + 0*\ybias) {$\acqSubs{2}{\ell_{\{1,2\}}}$};
\node[event, draw=black, fill=white] (22) at (2*\xstep, 2*\ystep + 0*\ybias) {$\acqSubs{2}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white] (23) at (2*\xstep, 3*\ystep + 0*\ybias) {$\writeOp{s_2}$};
\node[event, draw=black, fill=white] (24) at (2*\xstep, 4*\ystep + 0*\ybias) {$\readOp{z_2^1}$};
\node[event, draw=black, fill=white] (25) at (2*\xstep, 5*\ystep + 0*\ybias) {$\relSubs{2}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white] (26) at (2*\xstep, 6*\ystep + 0*\ybias) {$\relSubs{2}{\ell_{\{1,2\}}}$};
\node[event, draw=black, fill=white] (27) at (2*\xstep, 7*\ystep + 1*\ybias) {$\acqSubs{2}{\ell_{\{1,2\}}}$};
\node[event, draw=black, fill=white] (28) at (2*\xstep, 8*\ystep + 1*\ybias) {$\writeOp{y_2^2}$};
\node[event, draw=black, fill=white] (29) at (2*\xstep, 9*\ystep + 1*\ybias) {$\readOp{z_2^2}$};
\node[event, draw=black, fill=white] (210) at (2*\xstep, 10*\ystep + 1*\ybias) {$\relSubs{2}{\ell_{\{1,2\}}}$};
\node[event, draw=black, fill=white] (211) at (2*\xstep, 11*\ystep + 2*\ybias) {$\acqSubs{2}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white, line width=1.75] (212) at (2*\xstep, 12*\ystep + 2*\ybias) {$\writeOp{y_2^3}$};
\node[event, draw=black, fill=white] (213) at (2*\xstep, 13*\ystep + 2*\ybias) {$\readSubs{2}{x}$};
\node[event, draw=black, fill=white] (214) at (2*\xstep, 14*\ystep + 2*\ybias) {$\relSubs{2}{\ell_{\{1,3\}}}$};
\node[event, draw=black, fill=white] (302) at (2*\xstep, 15*\ystep + 2*\ybias) {$\writeOp{v_2}$};



\node[event, draw=black, fill=white] (31) at (1*\xstep, 4*\ystep + 1*\ybias) {$\acqUps{1}{\ell_1}$};
\node[event, draw=black, fill=white] (32) at (1*\xstep, 5*\ystep + 1*\ybias) {$\writeOp{z_1^1}$};
\node[event, draw=black, fill=white] (33) at (1*\xstep, 6*\ystep + 1*\ybias) {$\readOp{y_1^2}$};
\node[event, draw=black, fill=white, line width=1.75] (34) at (1*\xstep, 7*\ystep + 1*\ybias) {$\relUps{1}{\ell_1}$};
\node[event, draw=black, fill=white] (35) at (1*\xstep, 10*\ystep + 1*\ybias) {$\acqUps{2}{\ell_1}$};
\node[event, draw=black, fill=white] (36) at (1*\xstep, 11*\ystep + 1*\ybias) {$\writeOp{z_1^2}$};
\node[event, draw=black, fill=white] (37) at (1*\xstep, 12*\ystep + 1*\ybias) {$\readOp{y_1^3}$};
\node[event, draw=black, fill=white] (38) at (1*\xstep, 13*\ystep + 1*\ybias) {$\relUps{2}{\ell_1}$};
\node[event, draw=black, fill=white] (303) at (1*\xstep, 15*\ystep + 2*\ybias) {$\writeOp{v_3}$};

\node[event, draw=black, fill=white] (41) at (3*\xstep, 4*\ystep + 1*\ybias) {$\acqUps{1}{\ell_2}$};
\node[event, draw=black, fill=white] (42) at (3*\xstep, 5*\ystep + 1*\ybias) {$\writeOp{z_2^1}$};
\node[event, draw=black, fill=white] (43) at (3*\xstep, 6*\ystep + 1*\ybias) {$\readOp{y_2^2}$};
\node[event, draw=black, fill=white] (44) at (3*\xstep, 7*\ystep + 1*\ybias) {$\relUps{2}{\ell_2}$};
\node[event, draw=black, fill=white] (45) at (3*\xstep, 10*\ystep + 1*\ybias) {$\acqUps{2}{\ell_2}$};
\node[event, draw=black, fill=white] (46) at (3*\xstep, 11*\ystep + 1*\ybias) {$\writeOp{z_2^2}$};
\node[event, draw=black, fill=white] (47) at (3*\xstep, 12*\ystep + 1*\ybias) {$\readOp{y_2^3}$};
\node[event, draw=black, fill=white, line width=1.75] (48) at (3*\xstep, 13*\ystep + 1*\ybias) {$\relUps{2}{\ell_2}$};
\node[event, draw=black, fill=white] (304) at (3*\xstep, 15*\ystep + 2*\ybias) {$\writeOp{v_4}$};


\node[event, draw=black, fill=white] (51) at (4*\xstep, 7*\ystep + -0.2*\ybias) {$\writeOp{q}$};
\node[event, draw=black, fill=white] (305) at (4*\xstep, 15*\ystep + 2*\ybias) {$\writeOp{v_5}$};
\node[event, draw=black, fill=white] (312) at (4*\xstep, 16*\ystep + 2*\ybias) {$\writeSubs{1}{a}$};

\node[event, draw=black, fill=white] (61) at (5*\xstep, 4*\ystep + 0.25*\ybias) {$\readOp{s_1}$};
\node[event, draw=black, fill=white] (62) at (5*\xstep, 5*\ystep + 0.25*\ybias) {$\readOp{s_2}$};
\node[event, draw=black, fill=white] (63) at (5*\xstep, 6*\ystep +  0.25*\ybias) {$\acq{\ell_1}$};
\node[event, draw=black, fill=white] (64) at (5*\xstep, 7*\ystep +  0.25*\ybias) {$\acq{\ell_2}$};
\node[event, draw=black, fill=white] (314) at (5*\xstep, 8*\ystep +  0.25*\ybias) {$\readOp{q}$};
\node[event, draw=black, fill=white] (65) at (5*\xstep, 9*\ystep +  0.25*\ybias) {$\writeOp{x}$};
\node[event, draw=black, fill=white] (66) at (5*\xstep, 10*\ystep +  0.25*\ybias) {$\rel{\ell_2}$};
\node[event, draw=black, fill=white] (67) at (5*\xstep, 11*\ystep +  0.25*\ybias) {$\rel{\ell_1}$};
\node[event, draw=black, fill=white] (306) at (5*\xstep, 16*\ystep + 2*\ybias) {$\readOp{v_5}$};
\node[event, draw=black, fill=white] (307) at (5*\xstep, 17*\ystep + 2*\ybias) {$\readOp{v_4}$};
\node[event, draw=black, fill=white] (308) at (5*\xstep, 18*\ystep + 2*\ybias) {$\readOp{v_2}$};
\node[event, draw=black, fill=white] (309) at (5*\xstep, 19*\ystep + 2*\ybias) {$\readOp{v_3}$};
\node[event, draw=black, fill=white] (310) at (5*\xstep, 20*\ystep + 2*\ybias) {$\readOp{v_1}$};
\node[event, draw=black, fill=white] (311) at (5*\xstep, 21*\ystep + 2*\ybias) {$\writeSubs{2}{a}$};


\draw[post, out=180, in=-0, looseness=-0.4] (32) to (14);
\draw[post, out=0, in=180, looseness=-0.4] (18) to (33);
\draw[post, out=180, in=-0, looseness=-0.4] (36) to (19);
\draw[post, out=0, in=180, looseness=-0.4] (112) to (37);

\draw[post, out=180, in=-0, looseness=-0.4] (42) to (24);
\draw[post, out=0, in=180, looseness=-0.4] (28) to (43);
\draw[post, out=180, in=-0, looseness=-0.4] (46) to (29);
\draw[post, out=0, in=180, looseness=-0.4] (212) to (47);

\draw[post] (13) to (61);
\draw[post, out=0, in=180, looseness=-0.4] (23) to (62);

% \draw[post, out=0, in=180, looseness=-0.4] (51) to (65);

\draw[post, out=180, in=0, looseness=0.75] (65) to ($ (48) + (0, 2.05*\ystep) $) to ($ (214) + (-0.5*\xstep, -0.25) $) to (113);

\draw[post, out=180, in=0, looseness=0.9] (65) to ($ (48) + (0, -0.4) $)  to  (213);

\draw[post, out=0, in=180, looseness=0.9] (301) to ($ (303) + (0, -2.5) $)  to  (310);

\draw[post, out=0, in=180, looseness=0.9] (303) to ($ (302) + (0, -2) $)  to  (309);

\draw[post, out=0, in=180, looseness=0.9] (302) to ($ (304) + (0, -1.5) $)  to  (308);

\draw[post, out=0, in=180, looseness=0.9] (304) to ($ (312) + (0, -0.5) $)  to  (307);

\draw[post, out=0, in=180, looseness=-0.4] (305) to (306);

\draw[post, out=0, in=180, looseness=-0.4] (51) to (314);

%\draw[post, out=-20, in=160, looseness=0.4] (A7) to (B25);


\end{tikzpicture}
}
\caption{
Illustration of the o-poset $\OPoset_G$ given a graph $G$ and independent-set size $c=2$.
Edges represent orderings in $P$.
\ucomment{Don't copy the diagram as is. Remember there is something called as Self Plagiarism: https://dl.acm.org/journal/tods/SelfPlagiarismPolicy}
}
\label{fig:w1hardness}
\end{figure*}

==> figures/fig_RMQdemo.tex <==
%!TEX root=../main.tex

\begin{figure}
\centering
\begin{subfigure}[b]{0.5\columnwidth}
  \centering
  \includegraphics[scale=0.06]{figures/ShortestPathDemo.png}
  \caption{Demo of the direct edges}
  \figlabel{rmq_direct_edges}
\end{subfigure}
\begin{subfigure}[b]{0.45\columnwidth}
  \centering
  \execution{3}{
    \figev{2}{\acq(\lk)}
    \figev{2}{\wt(x)}
    \figev{2}{\wt(y)}
    \figev{2}{e_4}
    \figev{1}{\rd(x)}
    \figev{1}{\wt(z)}
    \figev{2}{\rel(\lk)}
    \figev{3}{\acq(\lk)}
    \figev{3}{\rd(z)}
    \figev{3}{\rel(\lk)}
    \figev{3}{\rd(x)}
    \figev{3}{e_{12}}
  }
\caption{Trace $\trace_3$}
\figlabel{rmq_demo}
\end{subfigure}
\caption{Given a trace $\trace_3$, Algorithm \ref{algo:getSuccessors} solves cycle detection. The red events in (a) are $\SSP{e_4}{e_{12}}$}
\figlabel{RMQ-ShortesePath-Demo}
\end{figure}

==> figures/fig_syncp_race.tex <==
%!TEX root=../main.tex

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.45\columnwidth}
	\centering
	\execution{3}{
		\figev{1}{\acq(\lk_1)}
		\figev{1}{\wt(x)}
		\figev{1}{\rel(\lk_1)}
		\figev{2}{\acq(\lk_2)}
    \figev{2}{\rd(x)}
    \figev{2}{e_6}
    \figev{2}{\rel(\lk_2)}
		\figev{3}{\acq(\lk_1)}
		\figev{3}{e_9}
		\figev{3}{\rel(\lk_1)}
	}
	\caption{Trace $\trace_2$}
	\figlabel{syncp_race_trace}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.45\columnwidth}
  \centering
	\execution{3}{
            \figev{1}{\acq(\lk_1)}
		\figev{1}{\wt(x)}
		\figev{1}{\rel(\lk_1)}
		\figev{2}{\acq(\lk_2)}
            \figev{2}{\rd(x)}
            \figev{3}{\acq(\lk_1)}
            \figev{2}{e_6}
            \figev{3}{e_9}
            \figev{2}{\rel(\lk_2)}
            \figev{3}{\rel(\lk_1)}
	}
	\caption{Witness $\reordering$}
	\figlabel{syncp_race_witness}
\end{subfigure}
\caption{Example of a sync-preserving race between $e_6$ and $e_9$}
\figlabel{demo_syncp_race}
\end{figure}


% \captionsetup[table]{labelformat=empty}
% \begin{figure}
%     \centering
%     \centering
% 	\begin{minipage}[t]{0.45\columnwidth}
% 		\centering
%             \setlength{\tabcolsep}{0.5mm}{
% 			\begin{tabular}{|c|ccc|}
% 				\hline $\,$ & $t_1$      & $t_2$    & $t_3$    \\
% 				\hline 1    & $\acq(\lk_1)$      & $\,$     & $\,$     \\
% 				2           & $\wt(x)$   & $\,$     & $\,$     \\
% 				3           & $\rel(\lk_1)$   & $ $      & $\,$     \\
% 				4           & $\,$       & $\acq(\lk_2)$ & $\,$     \\
% 				5           & $\,$       & $\rd(x)$    & $\,$     \\
% 				6           & $\,$       & $e_6$ & $\,$     \\
% 				7           & $\,$       & $\rel(l_2)$     & $ $ \\
% 				8           & $\,$       & $\,$     & $\acq(\lk_1)$   \\
% 				9           & $\,$       & $\,$     & $e_9$ \\
% 				10          & $\,$       & $\,$     & $\rel(\lk_1)$ \\
% 				\hline
% 			\end{tabular}
% 			\caption*{\textbf{(a)} Trace $\trace$}
%         }
% 	\end{minipage}
% 	\begin{minipage}[t]{0.45\columnwidth}
% 		\centering
%             \setlength{\tabcolsep}{0.5mm}{
% 			\begin{tabular}{|c|ccc|}
% 				\hline $\,$ & $t_1$      & $t_2$    & $t_3$    \\
% 				\hline 1    & $\acq(\lk_1)$      & $\,$     & $\,$     \\
% 				2           & $\wt(x)$   & $\,$     & $\,$     \\
% 				3           & $\rel(\lk_1)$   & $ $      & $\,$     \\
% 				4           & $\,$       & $\acq(\lk_2)$ & $\,$     \\
% 				5           & $\,$       & $\rd(x)$    & $\,$     \\
% 				6           & $\,$       & $ $       & $\acq(\lk_1)$     \\
% 				7           & $\,$       & $ $     & $ $ \\
% 				8           & $\,$       & $\,$     & $ $   \\
% 				9           & $\,$       & $\,$     & $ $ \\
% 				10          & $\,$       & $\,$     & $ $ \\
% 				\hline
% 			\end{tabular}
% 			\caption*{\textbf{(b)} Witness $\reordering$}
%             }
% 	\end{minipage}
%     \caption{Example of a $\syncp$ race between $e_6$ and $e_9$}
%     \label{fig:my_label}
% \end{figure}

% \captionsetup[table]{labelformat={default}}

==> figures/non-osr-races.tex <==
%!TEX root=../main.tex

\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.55\columnwidth}
	\centering
  \executionThin{5}{
    \figev{1}{\textcolor{red}{w(x)}}
    \figev{1}{\wt(z_1)}
    \figev{2}{\acq(\lk_1)}
    \figev{2}{\wt(z_2)}
    \figev{2}{\rel(\lk_1)}
    \figev{3}{\acq(\lk_1)}
    \figev{3}{\wt(z_3)}
    \figev{2}{\acq(\lk_2)}
    \figev{2}{\wt(z_4)}
    \figev{2}{\rd(z_1)}
    \figev{2}{\rel(\lk_2)}
    \figev{3}{\rd(z_4)}
    \figev{5}{\acq(\lk_2)}
    \figev{5}{\wt(z_5)}
    \figev{5}{\rd(z_1)}
    \figev{5}{\rel(\lk_2)}
    \figev{3}{\rd(z_5)}
    \figev{3}{\rel(\lk_1)}
    \figev{4}{\rd(z_2)}
    \figev{4}{\rd(z_3)}
    \figev{4}{\textcolor{red}{w(x)}}
  }
	\caption{SyncP Race, but not M2/OSR race}
  \figlabel{syncp-only-race}
\end{subfigure}  
\hfill
\begin{subfigure}[b]{0.4\columnwidth}
  \centering
  \executionThin{2}{
    \figev{1}{\wt(x_1)}
    \figev{1}{\wt(x_2)}
    \figev{1}{\wt(x_3)}
    \figev{1}{\acq(\lk)}
    \figev{1}{\wt(x_4)}
    \figev{1}{\rd(x_1)}
    \figev{1}{\rel(\lk)}
    \figev{1}{\acq(\lk)}
    \figev{1}{\rd(x_4)}
    \figev{1}{\textcolor{red}{w(x)}}
    \figev{1}{\rel(\lk)}
    \figev{2}{\wt(x_3)}
    \figev{2}{\acq(\lk)}
    \figev{2}{\wt(x_4)}
    \figev{2}{\rel(\lk)}
    \figev{2}{\wt(x_1)}
    \figev{2}{\rd(x_2)}
    \figev{2}{\rd(x_3)}
    \figev{2}{\textcolor{red}{\rd(x)}}
  }
    \caption{M2 Race, but not SyncP nor OSR race}
    \figlabel{m2-only-race}
\end{subfigure}
\hfill
\caption{Two traces containing two predictable races. One of them (a) can be detected by \syncp, but not M2 nor OSR. 
The other one (b) can be detected by M2, but not \syncp nor OSR. 
Trace in (b) is directly cited from M2 paper \cite{m2} without modification.
}
\figlabel{non-osr-races}
\end{figure}
